The Public Algorithms Survey in Allegheny County

This survey study focuses on public opinion regarding the use of algorithmic decision-making in government sectors, specifically in Allegheny County, Pennsylvania. Algorithms are becoming increasingly prevalent in various public domains, including both routine and high-stakes government functions. Despite their growing use, public sentiment remains divided, with concerns about privacy and accuracy juxtaposed against perceptions of fairness when compared to human decision-making. In April 2021, a survey was conducted among nearly 1,500 county residents to explore their awareness, experiences, and attitudes towards these algorithms. The study highlights diverse viewpoints influenced by factors such as race, age, education, gender, income, and urban or suburban living. The results demonstrate the complexity of public sentiment towards algorithmic governance and emphasize the need for a nuanced understanding and approach in policy and implementation.

==> figs/figA1.tex <==
\begin{figure}
\paragraph{Do you know of any algorithms that the City of Pittsburgh and Allegheny County uses to make or help make decisions in the public sector?}
  \includegraphics[width=1.4\linewidth]{Q01_all6demo}
  \caption{Awareness of the use of public algorithms.}
  \label{fig:Q1demo}
  \setfloatalignment{b}
\end{figure}

==> figs/figA2.tex <==
\begin{figure}
\paragraph{How did you become aware of these algorithms? (Select all that apply)}
  \includegraphics[width=1.4\linewidth]{Q01b_all6demo}
  \caption{Source of awareness.}
  \label{fig:Q1bdemo}
  \setfloatalignment{b}
\end{figure}


==> figs/figA3.tex <==
\begin{figure}
\paragraph{Below is a list of algorithms being developed, in-use, or previously in-use locally. Before taking this survey, which public algorithms have you heard about in the City of Pittsburgh or Allegh...?}
  \includegraphics[width=1.4\linewidth]{Q04_all6demo}
  \caption{Awareness of algorithms in use locally.}
  \label{fig:Q4demo}
  \setfloatalignment{b}
\end{figure}

==> figs/figA4.tex <==
\begin{figure}
\paragraph{What level of impact do public algorithms have on you (e.g. safety, health and finances) to your knowledge?}
  \includegraphics[width=1.4\linewidth]{Q02_all6demo}
  \caption{Impact of algorithms.}
  \label{fig:Q2demo}
  \setfloatalignment{b}
\end{figure}

==> figs/figA5.tex <==
\begin{figure}
\paragraph{How much do you agree with the following statements about the government’s use of algorithmic decision-making tools?
I am concerned with ...}
  \includegraphics[width=1.4\linewidth]{Q05_age_gen}
  \caption{Concerns about algorithms -- by age \& gender.}
  \label{fig:Q5demo}
  \setfloatalignment{b}
\end{figure}

\begin{figure}
\paragraph{How much do you agree with the following statements about the government’s use of algorithmic decision-making tools?
I am concerned with ...}
  \includegraphics[width=1.4\linewidth]{Q05_eth_edu}
  \caption{Concerns about algorithms -- by ethnicity \& education.}
  \label{fig:Q5demo}
  \setfloatalignment{b}
\end{figure}

\begin{figure}
\paragraph{How much do you agree with the following statements about the government’s use of algorithmic decision-making tools?
I am concerned with ...}
  \includegraphics[width=1.4\linewidth]{Q05_inc_loc}
  \caption{Concerns about algorithms -- by income \& residence.}
  \label{fig:Q5demo}
  \setfloatalignment{b}
\end{figure}

==> figs/figA6.tex <==
\begin{figure}
\paragraph{Governments should use algorithms in the following public sector(s):}
  \includegraphics[width=1.4\linewidth]{Q06_age_gen}
  \caption{Need of algorithms -- by age \& gender.}
  \label{fig:Q6demo}
  \setfloatalignment{b}
\end{figure}

\begin{figure}
\paragraph{Governments should use algorithms in the following public sector(s):}
  \includegraphics[width=1.4\linewidth]{Q06_eth_edu}
  \caption{Need of algorithms -- by ethnicity \& education.}
  \label{fig:Q6demo}
  \setfloatalignment{b}
\end{figure}

\begin{figure}
\paragraph{Governments should use algorithms in the following public sector(s):}
  \includegraphics[width=1.4\linewidth]{Q06_inc_loc}
  \caption{Need of algorithms -- by income \& residence.}
  \label{fig:Q6demo}
  \setfloatalignment{b}
\end{figure}

==> figs/figA7.tex <==
\begin{figure}
\paragraph{How much do you agree with the following statements about Pittsburgh City’s use of algorithmic tools?
There is enough \rule{1cm}{0.15mm} over government use of algorithmic tools.}
  \includegraphics[width=1.4\linewidth]{Q07_all6demo}
  \caption{Attitude toward City's use of algorithms.}
  \label{fig:Q7demo}
  \setfloatalignment{b}
\end{figure}

==> figs/figA8.tex <==
\begin{figure}
\paragraph{Do you interact with any of the following local government sectors? (Select all that apply)}
  \includegraphics{Q03_all}
  \caption{Interaction with government sectors.}
  \label{fig:Q3}
  \setfloatalignment{b}
\end{figure}




==> figs/figA9.tex <==
\begin{figure}
\paragraph{Do you interact with any of the following local government sectors? (Select all that apply)}
  \includegraphics[width=1.4\linewidth]{Q03_all6demo}
  \caption{Interaction with government sectors -- by demographics.}
  \label{fig:Q3demo}
  \setfloatalignment{b}
\end{figure}
